Model Cascading for Code: A Cascaded Black-Box Multi-Model Framework for Cost-Efficient Code Completion with Self-Testing

The rapid advancement of large language models (LLMs) has significantly improved code completion tasks, yet the trade-off between accuracy and computational cost remains a critical challenge. While using larger models and incorporating inference-time self-testing algorithms can significantly improve output accuracy, they incur substantial computational expenses at the same time. Furthermore, servers in real-world scenarios usually have a dynamic preference on the cost-accuracy tradeoff, depending on the budget, bandwidth, the concurrent user volume, and users' sensitivity to wrong answers. In this work, we introduce a novel framework combining model cascading and inference-time self-feedback algorithms to find multiple near-optimal self-testing options on the cost-accuracy tradeoff in LLM-based code generation. Our approach leverages self-generated tests to both enhance accuracy and evaluate model cascading decisions. As a blackbox inference-time method, it requires no access to internal model parameters. We further propose a threshold-based algorithm to determine when to deploy larger models and a heuristic to optimize the number of solutions, test cases, and test lines generated per model, based on budget constraints. Experimental results show that our cascading approach reduces costs by an average of 26%, and up to 70% in the best case, across various model families and datasets, while maintaining or improving accuracy in natural language generation tasks compared to both random and optimal single-model self-testing schemes. To our knowledge, this is the first work to provide a series of choices for optimizing the cost-accuracy trade-off in LLM code generation with self-testing.

==> figures/apps_result.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=8.5cm]{images/results/apps_wz_1_test_threshold0.9.pdf}
    \caption{WizardCoder-Python-V1.0 family on APPS-test introductory level subset. The setting is the same as all plots in Figure \ref{fig:all_test_pareto}.}
    \label{fig:apps_test_pareto}
\end{figure}


==> figures/equation_time.tex <==
\begin{figure*}[ht!]
\begin{equation*}
\begin{aligned}
% Acc_{1} &= acc_1 \ \ \ \ \ \ \ \ \ \ \ \  Acc_{2} = acc_2 \ \ \ \ \ \ \ \ \ \ \ \  Acc_{3} = acc_3\\
% Acc_{12} &= tp_1 
% + (tn_1 + fn_1) \cdot p_{12} \cdot \frac{acc_2^{k_2}}{acc_2^{0}} \\
% Acc_{13} &= tp_1 
% + (tn_1 + fn_1) \cdot p_{13} \cdot \frac{acc_3^{k_3}}{acc_3^{0}} \\
% Acc_{23} &= tp_2
% + (tn_2 + fn_2) \cdot p_{23} \cdot \frac{acc_3^{k_3}}{acc_3^{0}} \\
% Acc_{123} &= tp_1 
% + (tn_1 + fn_1) \cdot p_{12} \cdot \frac{acc_2^{k_2}}{acc_2^{0}} \cdot \frac{tp_2}{tp_2+fn_2}
% + (tn_1 + fn_1) \cdot (tn_2 + fn_2) \cdot p_{23} \cdot \frac{acc_3^{k_3}}{acc_3^{0}}\\ \\
Cost_{1} &= C_1 \ \ \ \ \ \ \ \ \ \ \ \ Cost_{2} = C_2 \ \ \ \ \ \ \ \ \ \ \ \ Cost_{3} = C_3 \\
Cost_{12} &= C_1 + (tn_1 + fn_1) \cdot C_2 \\
Cost_{13} &= C_1 + (tn_1 + fn_1) \cdot C_3 \\
Cost_{23} &= C_2 + (tn_2 + fn_2) \cdot C_3 \\
Cost_{123} &= C_1 + (tn_1 + fn_1) \cdot C_2 + (tn_1 + fn_1) \cdot (tn_2 + fn_2) \cdot C_3
\end{aligned}
\end{equation*}
\caption{This equation set illustrates the calculation of final accuracy (Acc) and final cost (Cost). Smallest to largest models are represented as 1,2,3. If we only use model 1 and model 3, for example, then $Acc_{13}$ and $Cost_{13}$ should apply. True/false positive/negative rates are represented as tp, tn, fp, fn. $p_{xy}$ means when looking at the greedy results of model x and model y, what is the percentage that y answers correctly among the questions that x answers incorrectly. So $p_{xy} = \frac{acc_y^0}{1-acc_x^0}$. $acc_x^{k}$ means the final accuracy of model x at pick@k. }
\label{fig:Cost-Accuracy Equations}
\end{figure*}


==> figures/time_accu_wz_he.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics{images/seed101_wc_he_val.png}
    \includegraphics{images/seed101_wc_he_test.png}
    \caption{Caption}
    \label{fig:time_accu_wz_he}
\end{figure*}

==> figures/train.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=9cm]{images/combinations/wizard_he_t1.0_val.png}
    \caption{WizardCoder-Python-V1.0 on HumanEval. Train set with 30\% of all questions, to select the pareto combinations. }
    \label{fig:train_example}
\end{figure}

==> figures/venn_wz_he.tex <==
\begin{figure}[hb!]
% \begin{figure}
    \centering
    \includegraphics[width=7cm]{images/venn_wz_he.pdf}
    \caption{Venn diagram of WizardCoder-Python-V1.0 models (7B, 13B, 34B) on answering HumanEval prompts using greedy search. Out of 164 prompts, numbers indicate questions correctly answered by one, two, or all three models. Examples: 21 by 13B and 34B, 2 only by 7B, 75 by all. 33 questions were unsolved by any model.}
    \label{fig:venn_diagram}
\end{figure}


==> settings.tex <==
% \usepackage[table]{xcolor}
% \usepackage[table, dvipsnames]{xcolor}
% \usepackage{color}
% \usepackage[table]{xcolor}
% \newcommand{\gray}{\cellcolor{gray}}
% \newcommand{\white}{\cellcolor{white}}
\usepackage{setspace}
% \setstretch{0.918}
% \settopmatter{printacmref=false,printccs=false,printfolios=true}
% \renewcommand\footnotetextcopyrightpermission[1]{}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{black}{#1}}
\newcommand{\black}[1]{\textcolor{black}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}

\newcommand{\new}[1]{\textcolor{blue}{#1}}
\renewcommand{\new}[1]{#1}
\usepackage{soul}
\newcommand{\drop}[1]{\textcolor{red}{#1}}
\renewcommand{\drop}[1]{}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\usepackage{multirow}
% \usepackage{color}
% \usepackage[table, dvipsnames]{xcolor}  % Modern color package (used for text and tables)
% \usepackage{xcolor}
\usepackage{enumitem}
% \settopmatter{printfolios=true}

% \usepackage{amsthm}% http://ctan.org/pkg/amsthm
\newtheorem{theorem}{Claim}

% \newtheorem{thm}{Theorem}
% \newtheoremstyle{exampstyle}
%   {\topsep} % Space above
%   {\topsep} % Space below
%   {} % Body font
%   {} % Indent amount
%   {\bfseries} % Theorem head font
%   {.} % Punctuation after theorem head
%   {.5em} % Space after theorem head


\usepackage{graphicx}
\usepackage{booktabs} 
% \usepackage{amsmath}
% \usepackage{tikz}
% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%             \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
% \usepackage{circledsteps}
% \usepackage{nicematrix}
\usepackage{pifont}
\usepackage{mathtools}
\def\smallerspacecaption{\vspace{-2mm}}

\usepackage[ruled, vlined, norelsize]{algorithm2e} % The algorithms writing package
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\SetKwInput{KwInit}{Initialization}
\SetKwInput{Kwprocedure}{Procedure}
\usepackage{lipsum}
\usepackage{dblfloatfix}

\usepackage{bm}

\newcommand{\todoj}[1]{\textcolor{red}{\textbf{Satwik:TODO:} #1}}{}

